Physics with high-luminosity proton-nucleus collisions at the LHC

The physics case for the operation of high-luminosity proton-nucleus ($pA$) collisions during Run 3 and 4 at the LHC is reviewed. The collection of $\mathcal{O}$(1-10 pb$^{-1}$) of proton-lead ($p$Pb) collisions at the LHC will provide unique physics opportunities in a broad range of topics including proton and nuclear parton distribution functions (PDFs and nPDFs), generalised parton distributions (GPDs), transverse momentum dependent PDFs (TMDs), low-$x$ QCD and parton saturation, hadron spectroscopy, baseline studies for quark-gluon plasma and parton collectivity, double and triple parton scatterings (DPS/TPS), photon-photon collisions, and physics beyond the Standard Model (BSM); which are not otherwise as clearly accessible by exploiting data from any other colliding system at the LHC. This report summarises the accelerator aspects of high-luminosity $pA$ operation at the LHC, as well as each of the physics topics outlined above, including the relevant experimental measurements that motivate -- much -- larger $pA$ datasets.

==> Complementarity-EIC-FT_LHC.tex <==

\subsection{Complementarity with EIC and FT-LHC}
\label{sec:comp}

{\it
Put here the x vs Q2 plot with EIC, FT@LHC, HL-LHC

pA data to be taken in FT mode: complementary in x for PDF; for GPD is UPC in FT mode (ask Laure), ...

What EIC will not be able to cover that pA HL-LHC (in terms of higher lumi or upgraded detectors) will cover ? 
}

\Remark{CAF}{Incorporate this here instead: As for other pA runs, with sufficient luminosity, it would be possible to study the A-dependence of $J/\psi$ UPCs for $p, O$ and Pb beams. This makes the A-dependence for $\rho_0$ UPCs for $p, O$, Xe and Pb also feasible by extension, as well as e.g. $\chi_c$ photoproduction for the first time, that can principally come from photon-photon but also pomeron-pomeron or pomeron-odderon mechanisms. \Remark{CAF}{suggest to move $\chi_c$ to Sec. 3.5}}

\begin{figure}[th]
\begin{center}
\includegraphics[width=0.4\textwidth]{indicative_x_q2.jpg}
%\setlength{\belowcaptionskip}{-10pt}
\caption{\footnotesize Accessible regions in $x$ and $Q^2$ for different colliders.  (Remake this)
}
\label{fig:xq}
\end{center}
\end{figure}


Access to physics in $pA$ collisions is complementary to that which can be done in $pp$ and $AA$ collisions at the LHC, in fixed-target collisions at the LHC, and at the EIC.
Fig.~\ref{fig:xq} shows how the production of an object of mass, $M$, at a given rapidity, $y$, translates into information on $x$ and $Q^2$.
In principle, the HL-LHC covers the largest kinematic region.  However, in practice all this is not accessible for two reasons.
Firstly, collisions between identical projectiles simultaneously sample partons at $x=Me^{\pm y}/\sqrt{s}$.
Except for rapidities close to zero, the partons can usually not be distinguished and thus only a narrow band in the plane is unambiguously accessible.
Secondly, the high-$x$ and low-$x$ regions, where much interesting physics such as saturation and the EMC-effect exist, are only accessible at very forward rapidities where detectors are poorly instrumented.

Photoproduction of vector mesons in $pA$ collisions with detectors instrumented up to pseudorapidities of 5 units access photon-nucleon centre-of-mass energies, $W$, from 6~GeV to 3~TeV, or equivalently $10^{-6}<x<0.1$.
For the EIC, $x$ is typically in the range 0.0002 to 0.2 and thus $pA$ collisions access much lower $x-$values with increased sensitivity to saturation effects.  On the other hand, electro-production and polarised beams is only possible at the EIC.
Probing $x-$values above about 0.1 can only be done in fixed-target collisions at the LHC.  Production of $J/\psi$ mesons in the LHCb SMOG system occurs for $0.075<x<0.44$ and will allow investigation of the EMC region. 

A summary of measurements achievable at each facility was given in Table~\ref{tab:comp_qual}.

The PDFs at relatively low-$Q^2$ are directly measured in inclusive neutral deep-inelastic scattering at the EIC.
Specific measurements in $pp$ collisions are sensitive in the same kinematic range but are more indirect since they always measure the convolution of two PDFs.  However, they uniquely probe the high-$Q^2$ region, most notably in $W$ and $Z$ production.  Photoproduction in $pA$ collisions probes a single PDF via the Shuvaev transform.

The workhorse for GPD extraction is deeply virtual Compton scattering (DVCS) that is only achievable at the EIC. However, the inverse process, time-like Compton scattering (TCS) can uniquely be measured in $pA$ processes~\cite{Pire:2008ea}.  Furthermore, GPDs are probed in exclusive photoproduction.

Nuclear PDFs can be constrained in $pA$ collisions as described in {sec:npdf}, while they can be accessed in electron-ion collisions at the EIC and at high-$x$ in FT-LHC.

Low-$x$ physics measurements allows searches for saturation.  When looking for saturation effects on the proton, the reach in $pA$ collisions is considerably better than at the EIC and is a cleaner environment than in $pp$ collisions.  Nuclear effects may enhance the onset of saturation that could be observed through changes in the momentum spectrum for photoproduced vector mesons: here the EIC and UPC $AA$ collisions are competitive. 

The odderon can be directly seen in C-even processes at the EIC~\cite{Benic:2024pqe} with high-luminosity running or in $pA$ or $AA$ collisions at the LHC~\cite{McNulty:2020ktd}.

Sufficient data likely exist for spectroscopy studies up to and including the charm threshold in $pp$ collisions.  However, photoproduction of such states can be cleaner and gives different information on the produced particle in $pA$ collisions, and much more data is needed here.







==> conclusions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
\label{sec:conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace*{-0.5cm}

In view of the forthcoming update of the European strategy for particle physics, this document promotes the physics case for an ambitious proton-nucleus programme at the LHC, and gathers the community in support of it. High-luminosity \pA\ collisions in Run 3 and Run 4 at the highest nucleon-nucleon CM energies of 8.54~TeV,  %\textcolor{red}{check} Yes with Ep = 6.8 TeV
involving both heavy and light nuclei, are essential to fully exploit a rich experimental program for the study of QCD in the perturbative, nonperturbative, and high-density regimes.
They provide, in particular, a unique and complementary environment for uncovering the tomography of the proton and nuclei, and their partonic properties.

Compared to \pp\ collisions, \pA\ interactions allow the exploration of nuclear modifications to PDFs and cold nuclear matter effects, which are essential for understanding the initial-state conditions of heavy-ion collisions. Additionally, \pA\ collisions probe small-$x$ physics more effectively than \pp, providing insight into gluon saturation and the onset of nonlinear QCD effects, which are enhanced due to the intrinsically larger number of initial partons.
%, but are easier to interpret than in AA collisions.

Unlike AA collisions, \pA\ collisions offer higher nucleon-nucleon CM energies, higher luminosity, and a cleaner environment, free from the final-state complexities of a fully-developed QGP, making them an essential benchmark for interpreting heavy-ion data, while studying the onset of collectivity in small systems. Photoproduction in \pA\ collisions, which capitalises on the LHC as a photon-collider, complements the UPC programme in AA collisions, and has many benefits through being able to distinguish the --more energetic-- photon emitter.  
%Additionally, \pA\ collisions probe small-$X$ physics more effectively than \pp\, providing insight into gluon saturation and the onset of non-linear QCD dynamics. 

%\old{Heavy-flavour and quarkonium studies in \pA\ collisions are particularly valuable, as they help disentangle initial- and final-state effects, improving our understanding from heavy-quark energy loss and nuclear effects, to exotic hadron formation. }
Investigations of quarkonium production, exotic hadrons, BSM scenarios, and hadronisation mechanisms, can all be performed in detail in an environment that bridges the gap between \pp\ and AA systems, and improves our understanding of ultrahigh-energy cosmic-ray interactions, underscoring the importance of \pA\ data in advancing our knowledge of high-energy nuclear, particle, and astroparticle physics. 
%
The data taken in \pA\ collisions at Run 1 and 2 of the LHC programme has had a major impact for all these fields, extrapolating precise knowledge of proton collisions to multi-nucleon systems.
The novel use of these collisions has brought significant advances to our understanding of both the proton and the nucleus. Run 3 is currently planned with only \pp\ and AA collisions: the absence of \pA\ collisions to date is notable and appears as a missed opportunity. We strongly encourage additional \pA\ running at the LHC in Runs 3 and 4, in order to achieve and extend the original physics targets, and to provide the data for the many important measurements summarised in this document.

%Overall, a complete proton-nucleus programme can certainly and fruitfully be  carried out at the LHC, with a great impact on the European and world-wide science in the near future.

%The physics opportunities offered by the LHC proton-nucleus mode can be summarised as follows :

%... ~\\

%... ~\\

%\Remark{CAF}{previous summary text from my section, use here instead}
%To summarise, high-statistics proton–nucleus collisions in Run3 and Run4, involving both heavy and light nuclei, are essential to fully exploit a rich experimental program uncovering the tomography of the proton. 
%$pA$ collisions,
%In particular, $p$Pb collisions at the highest energies of 8.16 TeV are needed to fully exploit the energy dependence of inclusive, exclusive and dissociative quarkonium production in UPCs. To this end, we restate the request described in the CERN Yellow Report~\cite{YR_WG5_2018}: 150~nb$^{-1}$ for both p-Pb and Pb-p configurations, in both Run 3 and Run 4, making a total of 300~nb$^{-1}$ for Run 3, and 300~nb$^{-1}$ for Run 4 \Remark{CAF}{these are the ALICE projections only, see Tab. 1}. This requested pPb luminosity described in the CERN Yellow Report~\cite{YR_WG5_2018} is essential to achieve quarkonium photoproduction in UPCs described in~\cite{Bylinkin:2022wkm}. This ensures ample statistics at the highest possible energies, extending existing and generating new interactions between the theoretical and experimental communities through the fruitful phenomenological programs that emanate, as discussed.


%Overall, a complete proton-nucleus programme can certainly and fruitfully be  carried out at the LHC, with a great impact on the European and world-wide science in the near future.



==> further.tex <==

\subsection{Going further}
%\vspace{-0.25cm}

\subsubsection{Magnetic and Electric Dipole Moments}
%\vspace{-0.3cm}

Until now, MDM and EDM of charm and beauty baryons % or $\tau$ leptons 
have been experimentally elusive.
%
%mostly because of their short lifetime, with decay lengths of few cm for $\sim1$\tev particles.
%
They play a special role in QCD since the heavy-quark mass brings simplifications due to heavy-quark symmetry. 
As such, direct MDM measurements of heavy baryons at few per-cent level would add new constraints for low-energy QCD calculations and will help discriminate between some model predictions~\cite{Sharma:2010vv,Dhir:2013nka,Faessler:2006ft}.
%,Bernotas:2012nz}.
%Among them, of particular interest are effective theory approaches based on the heavy quark limit.
%
%Searches for hadronic EDM of second and even third generation quarks, arising from flavour-diagonal \CP violation, strongly suppressed within the SM.
%As no finite EDM has been observed so far and no source of BSM CP violation is known, heavy flavour EDM provide an uncharted territory to search for BSM physics and give clues on specific flavor structure of new physics. 
%Indirect constraints on e.g. the charm EDM are rather weak, of order $4 \times 10^{-17}$ecm~\cite{Sala:2013osa}.
%Even at a moderate precision of $10^{-17}-10^{-18}$~$e$\cm would provide access the electroweak scale (1-10\tev)~\cite{Pospelov:2018}.
%
The possibility to measure the MDM and EDM of heavy and strange baryons at the LHC has been explored in recent years~\cite{Baryshevsky:2016cul,Burmistrov:2194564,Bezshyyko:2017var,Baryshevsky:2017yhk,Botella:2016ksl,Bagli:2017foe,Baryshevsky:2018dqq,Fomin:2018ybj,Fu:2018tbs}.
%
The idea relies on a bent crystal to extract protons from the LHC beam halo. 
These protons then hit a dense target and produce charged baryons that will then be channelled in bent crystals positioned in front of the
detector. 
The intense electric field between the crystal atomic planes induces a sizeable spin precession during the lifetime of the particle. 
The EDM, along with the MDM, can be determined by analysing the angular distribution of the decay particles.
%  
%

About $2.4\times10^{14}$ $p$ on target could be reached with three years of data taking after the installation during an LHC technical stop during Run 3, either with two weeks per year of dedicated detector running at $10^8 p$/s or with parallel detector operation at $10^7 p$/s. 
This would lead to MDM and EDM sensitivities of roughly $10^{-4}\div10^{-1}$ and $10^{-18}\div10^{-13}$, respectively~\cite{Bagli:2017foe}.
%
%This would lead to MDM and EDM sensivities as reported in Fig.~\ref{fig:mu_delta_phys_reach} (S1 scenario).
%
Extending the detector coverage down to 10~mrad along with an increase of the proton flux during LHC Runs 4 and 5, either at LHCb or at a dedicated experiment, would improve sensitivity by about one order of magnitude, challenging the physics of and beyond the SM. 

\vspace{-0.35cm}
\subsubsection{Opportunities with secondary beams}
\vspace{-0.3cm}

If a dedicated beam line fed by bent-crystal extraction were to be built,
TeV secondary beams of $\pi$, $K$ could be created by impinging 7 TeV $p$ beam on a
primary target. The $\pi N$ DY COMPASS program~\cite{Chiosso:2013ila} has lately re-emphasised
the importance of pion-beam facilities to measure the Boer-Mulders functions. 
Meson beams are particularly interesting owing to their valence antiquark. 
Beyond meson beams, $e^+/e^-$  tertiary beams with an energy up to 4 TeV
could be considered~\cite{Uggerhoj:2005xz} with an efficiency up to $10^{-5}$.
The creation of hundred-GeV neutrino beam is another option to be explored
despite the likely significant civil engineering. It would allow for $\nu$ DIS studies 
at small $x$ (see~\cite{Adams:2009mc}).

\vspace{-0.35cm}
\subsubsection{Diffraction studies and forward detectors}
\vspace{-0.3cm}

As mentioned above, the Pb beam can be used as an effective photon source to study photoproduction process. 
It can also be used to study the diffractive dissociation of the proton into three jets and tests of colour transparency~\cite{Frankfurt:2002gb}.  

Most of the above physics discussion focused on the physics reach with detector 
covering up to $\eta_{\sf lab.}\sim$ 5. In the case of $pH$, $pA$ and Pb$H$ collisions, it is possible
to instrument the more forward region with roman pots to strengthen the physics case for exclusive and diffractive studies. 
This may allow one for instance to improve the tagging of UPCs by looking at forward neutron emissions or
to make sure that the colliding particles remained intact after the scattering. The corresponding feasibility studies
remain to be done. In the case of LHCb, the HeRSCheL detector may offer new physics opportunities yet unexplored.

\vspace{-0.35cm}
\subsubsection{Beyond unity}
\vspace{-0.3cm}

The domain $x >1$ in a nuclear target, which can be accessed in the most backward region, 
can probe specific aspects of the nuclear wavefunction such as the hidden-color excitations 
of the deuteron~\cite{Matveev:1977xt,Brodsky:1983vf} effectively corresponding to
six-quark Fock states. With liquid or gaseous deuteron targets, one can probe these 
in inclusive reactions requiring high 
$x$ ($ \geq 1 $) and by studying the diffractive dissociation of the deuteron
 in its rapidity domain~\cite{Akhieser:1957zz} in Pb$d$ collisions. In Pb$d$ UPCs, 
one could also measure the deuteron GPDs\cite{Berger:2001zb}.

Gluon and heavy-quark distributions are essentially unknown for $ x \geq 1 $ (see~\cite{Brodsky:2018zdh} for a recent theory 
study for the deuteron). Their study for deuterium or helium targets is clearly challenging 
but would give us new means to probe $n>3$ partonic Fock states in light nuclei and thus the strong interaction in these systems.

\vspace{-0.35cm}
\subsubsection{Multiply-heavy baryons}
\vspace{-0.3cm}
Similar to the {\it leading-particle} effect for light quarks, the possibility for IC
in the proton can lead to an excess of charmonium production at large $x$.
Along the same lines, the kinematics of the FT mode coupled with large luminosities 
and very good detector PID, may lead to the detections of very heavy baryons such as $\Omega_{ccc}$, $\Omega_{bbb}$, $\Xi^+_{ccb}$, ...,  
as well as single and double heavy-quark meson production such as $B_c$ 
in diffractive and non-diffractive channels. 
Such studies may be crucial to clear up the long-standing debate about the production mechanism of double-charm  baryons and their nature: 
the FT-based SELEX collaboration found what is considered to be the $\Xi_{cc}^+$~\cite{Mattson:2002vu,Ocherashvili:2004hi}, which however
was neither seen in $e^+e^-$ reactions by Babar~\cite{Aubert:2006qw} nor in the collider mode by LHCb~\cite{Aaij:2013voa} and the mass splitting between the $\Xi_{cc}^+$ and the $\Xi_{cc}^{++}$ recently discovered by LHCb \cite{Aaij:2017ueg} challenges many models.


\vspace{-0.35cm}
\subsubsection{Beyond the LHC}
\vspace{-0.3cm}	

The FT mode with future UHE hadron machines like the HE-LHC, the SppC and the FCC-hh has been discussed in the context of high luminosity studies of W$^\pm$, $Z^0$ and $H^0$ production at cms energies from 176 to 307 GeV~\cite{Lansberg:2015pra,Dainese:2016gch}. 
Correspondingly the boost between the laboratory and the cms frame ranges between 94 and 163 with a rapidity shift between 5.2 and 5.8. 
This energy range corresponds to that of RHIC and would certainly allow one to pursue QCD studies initiated at RHIC in the coming decades.
It is thus important not to reproduce the current situation of the LHC for which no FT program was planned, neither during the machine nor the detector designs.
 


\vspace{-0.35cm}
\subsubsection{Rapidity target studies}
\vspace{-0.3cm}

Accessing the entire backward hemisphere (in the cms system) at the LHC in FT mode, together with precise DY measurements, would allow one to study the target fracture functions~\cite{Ceccopieri:2015rha}. Measuring recoil particles may also allow to measure missing masses to select (quasi-)elastic scatterings.
In addition, the good PID in the target region will allow one to study the limiting fragmentation (or extended longitudinal scaling) and cumulative effects, both examples of enhancements of particle production on nuclear targets at large $x$, which extend into regions which are kinematically forbidden in scattering on free nucleons.

%\comm{keywords: extended longitudinal scaling = limiting fragmentation; cumulative effects}

%\comm{Check slides JPL sent by email. Cite white papers from RHIC collaborations \cite{Back:2004je}.}



\clearpage


==> heavy-ion.tex <==

\subsection{Heavy-ion physics}
%\vspace*{-0.25cm}

Despite the considerable progress achieved in the last decades to understand the hadronic-matter properties at extreme conditions, key aspects remain challenging~\cite{LRP2017}. 
The clarification of crucial properties of the QCD phase structure requires a facility to study HIC spanning energy and rapidity regimes not covered by the existing $AA$, $pA$ and $pp$ programmes. 
This is the scope of the FTP4LHC HIC research axis, in which we propose to measure, at an energy between RHIC and SPS:\\
(i) The suppression of the entire bottomonium family.\\
(ii) A complete set of charm observables down to low $P_T$ (e.g. $\psi$, $\chi_c$, $D$, $D+D$, $\psi+D$ and their ratios), complemented by bottom production observables.\\
(iii) The DY process in $p$A, Pb$p$ and PbA collisions to check --for the first time-- the collinear factorisation in HIC.\\
(iv) Particle yields and azimuthal asymmetries over the entire negative $y_{\sf cms}$ to perform a {\it rapidity scan} complementary to the {\it beam-energy scan} of RHIC whose primary goals are to probe the temperature dependence of the shear viscosity and look for the QCD critical point.
%\begin{enumerate}
%\item[(i)] The suppression of the entire bottomonium family.
%\item[(ii)] A complete set of charm observables down to low $P_T$ (e.g. $\psi$, $\chi_c$, $D$, $D+D$, $\psi+D$ and their ratios), complemented by bottom production observables.
%\item[(iii)] The DY process in $p$A, Pb$p$ and Pb$A$ collisions to check --for the first time-- the collinear factorisation in HIC.
%\item[(iv)] Azimuthal asymmetries over the entire negative $y_{\sf cms}$ to perform a ``rapidity scan'' complementary to the ``beam-energy scan'' of RHIC whose primary goals are to probe the temperature dependence of the shear viscosity and look for the QCD critical point.
%\end{enumerate}


As for charmonia, the precision data will be sufficient to greatly contribute to the resolution of the long-standing charmonium-suppression puzzle~\cite{Andronic:2015wma,Brambilla:2010cs,Rapp:2008tf}. \cf{figa:heavy-ion} shows the projected statistical precision of the $J/\psi$ and $\psi(2S)$ nuclear modification factor vs $y_{\sf lab.}$ in PbXe ($R_{\sf PbXe}$) and $p$Xe ($R_{p{\sf Xe}}$) collisions in the FT mode.
% using the integrated luminosities $\int \mathcal L_{pp}$ = 250 pb$^{-1}$, $\int \mathcal L_{pXe}$ = 2 pb$^{-1}$, and $\int \mathcal L_{\sf PbXe}$ = 30 nb$^{-1}$ which fits in one month of Pb ion run~\cite{Trzeciak:2017csa}. 
%To isolate the quarkonium peaks have used, as usual, a uncorrelated-background subtraction procedure using the like-sign technique. 
It clearly shows that the per-cent level precision is within reach for the LHCb detector. 
Similar performances are expected with the ALICE muon arm owing to the background reduction from the absorber. Such measurements along with
$\chi_c$ and open HF ones  should allow one to uncover the charmonium sequential pattern predicted by Matsui and Satz more than 30 years ago~\cite{Matsui:1986dk}. 
Moreover, the 3 $\Upsilon(nS)$ states will be measurable~\cite{Hadjidakis:2018ifr,Trzeciak:2017csa,Massacrier:2015qba}, complementing the CMS LHC collider studies. 
These hinted at a sequential suppression, whose interpretation however remains unclear with the recent observation of a similar relative $\Upsilon(nS)$ suppression in $p$Pb collisions~\cite{Andronic:2015wma}. 
The FTP4LHC will address this issue.

The study of QCD collective effects is another domain where the FTP4LHC can have a considerable impact. \cf{figb:heavy-ion} displays the projected statistical uncertainties for the elliptic flow ($v_2$) measurements for identified hadrons using as low as 10 million 20-30\% central PbPb events, \ie\ for an integrated luminosity of 14/$\mu$b with the ALICE CB and LHCb detectors. Altogether, they could cover as much as 6 units of rapidity! 
This clearly indicates the reach for $v_2$ (and $v_n$ in fact~\cite{Hadjidakis:2018ifr}) precision studies over a very broad rapidity range. These will then yield to an accurate determination of the temperature dependence of the shear viscosity to entropy ratio $\eta/s$ complementing existing $v_n$ studies. %In particular, it will provide novel detailed constraints on the system evolution --including its transverse and longitudinal dynamics-- between SPS and the top RHIC energy. 

\cf{figc:heavy-ion} shows how a {\it rapidity scan} at 72~GeV can complement the RHIC {\it beam-energy scan} from 62.4~GeV down to 7.7~GeV for $y_{\sf cms}$ close to zero, and help us better understand the interplay between the baryon chemical potential $\mu_B$, the temperature $T$ and the rapidity. 
In fact, recent calculations show~\cite{Begun:2018efg,Karpenko:2018xam} that, in PbPb collisions in the LHC FT mode, $\mu_B$ does vary with rapidity in the range accessible by ALICE and LHCb. 
This $\mu_B$ range covers a large fraction of that accessible at the RHIC BES program~\cite{Aggarwal:2010cw}. 
Correlation and fluctuation measurements of conserved quantities in small rapidity bins provide new ways to search for the QCD critical point and to probe the nature of the phase transition to confined partons. 
%However, the interpretation of such data could be challenging since the origin of the $\mu_B$ rapidity dependence is an open question.
The large rapidity coverage of the LHC FT mode, combined with the excellent particle identification capabilities of ALICE and LHCb, makes it a perfect place for such a rapidity scan.

Finally, the LHC in the FT mode offers a unique playground to probe initial-state effects on quarks via DY measurements in different collision species. This will allow one to check whether such initial-state effects in $AA$ collisions, usually embedded in nuclear PDF defined within the collinear factorisation, can be extrapolated from $pA$ and $eA$ collision data. 
One indeed usually assumes that they linearly factorise, although some effects~\cite{Kopeliovich:2010mx}  may break this linearity. 
DY measurements in $AA$ collisions will be accessible in the backward region thanks to a smaller background compared to the collider mode~\cite{Trzeciak:2017csa}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering\captionsetup[subfloat]{width=0.95\columnwidth}\vspace*{-.25cm}
\subfloat[Projected statistical precision of $R_{\sf PbXe}$ and $R_{p{\sf Xe}}$ vs $y_{\sf lab.}$ for $\psi(nS)$ using LHCb in the FT mode
~\cite{Trzeciak:2017csa,Hadjidakis:2018ifr}.]{\includegraphics[width=0.75\columnwidth]{psiRaa_PbXe.pdf}\label{figa:heavy-ion}}\\\vspace*{-.25cm}
\subfloat[Projected statistical precision for elliptic flow measurements of various light hadrons vs $\eta_{\sf lab.}$ with the ALICE CB and the LHCb detectors used in the FT mode~\cite{Hadjidakis:2018ifr}.]{\includegraphics[width=0.75\columnwidth]{v2-PbPb72GeV-20-30centralEvents.pdf}\label{figb:heavy-ion}}\\\vspace*{-.25cm}
\subfloat[Illustration of the similarity between a beam-energy scan at RHIC and a rapidity scan in the LHC FT mode in terms
of values of T and $\mu_B$ probed~\cite{Begun:2018efg}.]{\includegraphics[width=0.75\columnwidth]{muB_vs_T_HRG_72GeV.pdf}\label{figc:heavy-ion}}
\vspace{-0.2cm}
\caption{
\footnotesize
Representative projections of the heavy-ion FTP4LHC.}
\label{fig:heavy-ion}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







\clearpage




==> high-x.tex <==

\subsection{High-$x$ frontier for particles and astroparticles}
%\vspace*{-.25cm}	

The FTP4LHC high-$x$ axis addresses long-standing puzzles such as the origin of the nuclear EMC effect in nuclei or a possible non-perturbative intrinsic charm or beauty content in the proton at high $x$.
Collecting such FT data will allow one to drastically reduce the uncertainty of the nuclear gluon distribution; 
this is imperative to use hard probes of the Quark-Gluon Plasma (QGP). A similar reduction in the proton case will directly
benefit searches of new heavy particles at hadron colliders (LHC, HE-LHC, FCC-hh).
With an extensive coverage of the backward region ($y_{\sf cms}<0$) corresponding to high $x$ in
the target, FTP4LHC is probably the best for such physics with hadron beams, complementing the scope of the US EIC.

\cf{fig:high-x1} clearly displays the impact of $pp$ Drell-Yan (DY) pair data, taken in the FT mode using LHCb, on the proton $u$-quark PDF.
We see a remarkable uncertainty reduction at high $x$; a similar effect is also observed for the nuclear valence PDFs for the $p$Xe case~\cite{Hadjidakis:2018ifr}.
As said above, a better determination of high-$x$ PDFs can be crucial for future searches for new heavy particles. 
Moreover, improved measurements of the $d/u$ PDF ratio for $x\to 1$ can tell which picture is valid among an SU(6) symmetric one where $d/u \to 1/2$, the dominance of a quark-scalar diquark where $d/u \to 0$, quark-hadron duality where $d/u \to 0.42$ or a simple perturbative QCD one where $d/u \to 1/5$. Imposing direct constraints on PDFs at such high $x$ are challenging but they will certainly shed new light on the transition between the inclusive and exclusive  regimes of QCD. For instance, the observation of HT corrections would signal correlations between valence quarks and thus give us information on their confinement.


Due to the large boost between the laboratory and cms frames, the LHC FT mode is the ideal set-up to uncover a non-perturbative excess of charm at high $x$, referred to as intrinsic charm (IC).
\cf{fig:high-x2} clearly illustrates this with expected deviations --as large as a factor of 5-- in inclusive-$D^0$-meson production.
The projected uncertainties, even up to $P_T \simeq 15$ GeV, are sufficient to pin down IC or to constrain it by up to an order of magnitude.
This is truly important to compute atmospheric-neutrino fluxes, which are the main background for the observation of e.g. the cosmic neutrinos in the PeV range seen by IceCube~\cite{Aartsen:2016ngq}.


The FTP4LHC also comprises unique studies of the high-$x$ nuclear gluon PDF --the least known nuclear PDF (nPDF). 
Let us highlight HF production, shown in \cf{fig:high-x3} for $B^\pm$ production in $p$Xe collisions with LHCb.
A significant reduction of the nPDF uncertainty in the EMC region is expected to be seen, similar to that observed in the shadowing region in the collider mode~\cite{Kusina:2017gkz}. 
In such data, final-state effects may come into play.
Yet, the study of the mass and $P_T$ dependence of HF production should allow one to separate them out from the initial-state nPDF ones.
The antishadowing flavour dependence can also be studied~\cite{Kovarik:2010uv}.
Finally, off-shell $W$ could be detected with luminosities of 10~fb$^{-1}$, providing data at high $x$ and reasonably large scales in a poorly known region with limited HT contamination.



Predicting the cosmic $\bar{p}$ spectrum requires knowing their production cross section for different nuclear channels and kinematics~\cite{Donato:2017ywo, Korsmeier:2018gcy}. 
The first LHCb FT data~\cite{Aaij:2018svt} showed the discriminating power between current cross-section parametrisations ~\cite{Korsmeier:2018gcy}. 
For $E_{\bar p} > 10$~GeV, theory still exhibits 20\% uncertainties for the $\bar{p}$ flux which increase fast at lower $E_{\bar p}$~\cite{Korsmeier:2018gcy}. 
Studies with ALICE of slow $\bar p$ (below few GeV) will thus complement the LHCb ones. 
Indeed, cosmic $\bar p$ data are extremely precise~\cite{Aguilar:2016kjl} at small $E_{\bar p}$ and will be even more so with the GAPS experiment~\cite{Ong:2017szd}. 
Collecting positrons and gamma-ray cross sections\cite{Salati:2010rc} is also of interest and is possible with ALICE and LHCb in the FT mode.
Let us add that the ALICE CB can measure large $E_{\bar p}$, close to the beam energy, in the inverse kinematics when the slow $\bar{p}$ emitted by the target is seen from the projectile rest frame as an ultra-fast one.
%
%Interpreting galactic cosmic-ray (CR) data requires both a correct source and magnetic-turbulence-spectrum modelling, and the knowledge of many cross sections regulating the production and destruction of relativistic particles interacting with the interstellar medium. 
%In many cases, data are scarce or missing. 
%Antimatter CRs, such as $\bar p$, $e^+$ and $\bar d$, are of particular interest to look for dark matter annihilations~\cite{Salati:2010rc}. 
Moreover, light-nuclei-production cross sections are also needed for galactic-transport-model calibration~\cite{Genolini:2018ekk}.  These can in principle be measured by the ALICE CB.



% Studying the so-called high-$x$ physics also provides us with novel decisive means to advance our experimental
% knowledge of the still poorly understood confinement properties of the strong interaction, which is one of the last
%  open questions about the Standard Model. Indeed, studying 
% high-$x$  fluctuations of a nucleon, where a single gluon carries the majority of the confined-system momentum,
% certainly tests QCD in a new limit never explored before.



% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.30\textwidth]{DY_pA_reweighting.pdf}
% \includegraphics[width=0.30\textwidth]{pt-ratio-3y4-150918.pdf}
% \includegraphics[width=0.30\textwidth]{charm_Rg_MU2GeV_xlin_90CL-crop.pdf}
% \includegraphics[width=0.30\textwidth]{antiproton-ALICE-2.pdf}
% \caption{}
% \label{fig:high-x}
% \end{figure}

\begin{figure}[!hbt]\vspace*{-.25cm}	
\centering \captionsetup[subfloat]{width=0.95\columnwidth}
\subfloat[\footnotesize $u$-quark PDF uncertainty projection after including DY-pair production pseudo-data.
The CT14 PDFs~\cite{Dulat:2015mca} were used and the projections were done using
the profiling method~\cite{Paukkunen:2014zia,Alekhin:2014irh}.]
{\includegraphics[width=0.3\textwidth]{DY_pp_modified.pdf}
\label{fig:high-x1}}\\\vspace*{-.25cm}	
\subfloat[\footnotesize 
Impact of the charm PDF uncertainty on the $D^0$ yield vs. $p_T$
compared to projected uncertainties. 
The orange and blue zones correspond to yields computed with IC PDFs~\cite{Pumplin:2005yf,Pumplin:2007wg}
The dashed-red curves indicate the $\mu_F$ uncertainty on the ``no-IC'' yield.]
{\includegraphics[width=0.3\textwidth]{pt-ratio-3y4-150918_modified.pdf}
\label{fig:high-x2}}\\\vspace*{-.25cm}	
\subfloat[Relative uncertainties of the gluon in Xe ($R_g^{Xe}$) at $\mu_F=2$~GeV in the nCTEQ15 nPDFs~\cite{Kovarik:2015cma} before (red) and after reweighting using $B^\pm$ $pp$ and $p$Xe pseudo-data.]
{\includegraphics[width=0.3\textwidth]{Bp_Rg_MU2GeV_xlin_90CL-crop.pdf}
\label{fig:high-x3}}
% \subfigure[~]{\includegraphics[width=0.4\textwidth]{antiproton-ALICE-2.pdf}
% \label{fig:high-x4}}
\vspace{-0.2cm}
\caption{%
%
\footnotesize{
Representative projections of the high-$x$ FTP4LHC.}
%
% Systematic uncertainties of 5\% are included and the statistical uncertainty for the
% background subtraction is assumed to be negligible which is reasonable assuming
% LHCb-like performances, see~\cite{LHCb:2017qap}. The rates were computed by assuming
% an average efficiency of $\langle \varepsilon \rangle = 10\%$ and $\BR(D^0 \to K\pi)=3.93 \%$.
%
}
\label{fig:high-x}
\end{figure}



\clearpage




==> spin.tex <==

\subsection{Spin and 3D nucleon structure}
%\vspace*{-0.25cm}

The spin part of the FTP4LHC bears on two pillars: STSA measurements with a polarised target and azimuthal-modulation studies. 
Both allow one to investigate the tri-dimensional (3D) complexity of partons confined in hadrons, and help unravel how quarks and gluons are bound in a spin-$1/2$ nucleon.
%Moreover, these measurements in hadron-hadron collisions are complementary to analogous studies in lepton-hadron reactions since, contrary to usual PDFs, some of the hadronic quantities involved (transverse-momentum-dependent functions) are not universal. 
In particular, DY STSA measurements will contribute to the worldwide effort towards the verification of the Sivers-asymmetry~\cite{Sivers:1989cc} sign change~\cite{Collins:2002kn,Brodsky:2002cx} between DY and semi-inclusive deep-inelastic scattering (SIDIS).
Corresponding extractions in the gluon sector would simply be ground-breaking owing to their expected precision. 
In addition, looking for azimuthal modulations in DY and pair-particle production will provide novel ways to study the correlations between the parton momentum and their own spin.


\cf{fig:spin1} shows two theoretical predictions of the DY STSA ($A_N$) compared to the projected statistical precision using the LHCb in the FT mode.
This can clearly put strict constraints on the quark Sivers effect and the related 3-parton correlation functions~\cite{Efremov:1981sh,Qiu:1991pp}, help discriminate among different approaches, and test the time-reversal symmetry of QCD, realised through the relevant initial/final state interactions for DY and SIDIS.
We note how crucial it is to be able to access the rapidity region $2 < y_{\rm lab} <3$ to access the high $x^\uparrow$ region~\cite{Kikola:2017hnp}.
In addition, as shown in \cf{fig:spin2}, the projected statistical precision for several other asymmetries in DY production is expected to be as good as a few percent.
They would for the first time offer the opportunity to constrain even less known transverse-momentum distributions, such as $h_1^q$, $h_1^{\perp q}$ and $h_{1T}^{\perp q}$, which encapsulate more information on the quark-hadron momentum-spin correlations, and thus indirectly on the quark orbital angular momentum (OAM) (see \cite{Hadjidakis:2018ifr} for more details).

Besides, a major strength of the LHC FT mode is the large production rates for open heavy-flavour mesons and quarkonia (roughly $10^6$ $\Upsilon$ and $10^9$ $J/\psi$ for a single year of data taking~\cite{Massacrier:2015qba,Feng:2015rka}).
These processes are very useful probes to precisely access and constrain the gluon Sivers effect, still essentially unknown~\cite{Boer:2015vso}.
For instance, \cf{fig:spin3} shows the projected statistical precision with ALICE in the FT mode for $\jpsi$ $A_N$, compared to the existing measurements~\cite{Adare:2010bd,Aidala:2018gmp} and theoretical predictions~\cite{DAlesio:2017rzj}.



\begin{figure}[!hbt]
\centering\captionsetup[subfloat]{width=0.95\columnwidth}
\subfloat[Two predictions (AD'AM~\cite{Anselmino:2015eoa} and EIKV~\cite{Echevarria:2014xaa}) of the DY $A_N$ at LHCb in the FT mode, compared to the projected precision of the measurement~\cite{Kikola:2017hnp}. 
Bands are filled in the region where the fits use existing SIDIS data and hollow where they are extrapolations.]
{\includegraphics[width=0.4\textwidth]{AnDY-pp115GeV-L10invfb-models-v3}
\label{fig:spin1}}\\
\subfloat[Projected statistical uncertainty on asymmetries in DY production with LHCb (the rapidity is integrated over, as well as the mass in bins of $dM=1$~GeV/$c^2$).]
{\includegraphics[width=0.34\textwidth]{DY_AN_uncertainty_y3p4.pdf}
\label{fig:spin2}}\\
\subfloat[Projected precision for $J/\psi$ $A_N$ compared to existing measurements~\cite{Adare:2010bd,Aidala:2018gmp} using the ALICE Muon Spectrometer. 
%Signal and background are extrapolated at $\sqrt{s_{NN}}=115$~GeV from ALICE measurements~\cite{Adam:2015rta}.
]
{\includegraphics[width=0.42\textwidth]{AnJpsi-statErr-ALICE-L45inv-pb-3-12-2018.pdf}
\label{fig:spin3}}
\vspace{-0.2cm}
\caption{
\footnotesize{
Representative projections of the spin FTP4LHC.
}}
\label{fig:spin}\vspace*{-0.5cm}
\end{figure}

Ultraperipheral collisions in the FT mode~\cite{Lansberg:2015kha} offer access to photoproduction in hadron-hadron interactions~\cite{Baltz:2007kq}. 
Such exclusive reactions can help study the 3D ``tomography'' in position space of hadrons in terms of generalised parton distributions (GPDs)~\cite{Diehl:2003ny, Belitsky:2005qn,Radyushkin:1997ki,Ji:1996nm,Mueller:1998fv}, directly related to the parton OAM.
It remains to be studied whether additional detectors will be required to trigger on these exclusive reactions.
%They also allow one to explore the 3D ``tomography'' of hadrons~\cite{Burkardt:2000za}.
In particular, Timelike Compton Scattering~\cite{Berger:2001xd}, via lepton-pair photoproduction~\cite{Lansberg:2015kha} and $\jpsi$ photoproduction~\cite{Lansberg:2018fsy}, might provide additional information on GPDs.

Finally, at the LHC in the FT mode one can also access the distributions of longitudinally polarised (anti)quarks inside a nucleon, which are not well known (see e.g.~\cite{Nocera:2014gqa}), through the measurement of the longitudinal spin transfer $D_{LL}$ from a longitudinal polarised target to $\Lambda$ or $\bar{\Lambda}$ hyperons, for which only limited experimental results exist~\cite{Abelev:2009xg,Alekseev:2009ab,Adam:2018kzl}.
Specifically, the understanding of the distribution of polarised strange and anti-strange quark distributions, and their possible asymmetry, is a very intriguing open question in hadronic physics. 
Moreover, similar measurements can be carried out for the transverse spin transfer $D_{TT}$ to hyperons, with a similar precision to that for $D_{LL}$, giving access to the integrated quark transversity (also called the nucleon tensor charge).
This quantity is a useful input in the search for new physics and is now studied on the lattice~\cite{Chang:2017eiq}.
In general, any additional data at high $x$ can reduce the uncertainties in the determination of (un)polarised parton distributions, so the FTP4LHC can provide unmatched opportunities for such studies.

\clearpage




==> summary.tex <==
\clearpage

\section{Executive Summary}

High-energy proton-nucleus collisions (\pA) provide a bridge between proton-proton (\pp) and ion-ion (AA) collisions with two particular merits: firstly, the asymmetric projectiles and beam energies ensure that effects associated with the proton can be distinguished from those of the nucleus; secondly, a path towards understanding the complexity of two large systems of bound nucleons colliding is provided through interaction of a well-understood proton on the complex ion.

At the LHC, a few weeks of \pA\ collisions were performed in Runs 1 and 2 in a diversity of operating conditions, and have already brought essential contributions to particle, heavy-ion, and cosmic-rays physics,
%Limited operation with \pA\ collisions has been performed in Runs 1 and 2 at the LHC, and has already brought essential contributions to particle and heavy-ion physics, 
leading to the discovery of new phenomena as well as the confirmation and extension of effects discovered in lepton-nucleus collisions. Multi-TeV \pA\ collisions offer several unique physics opportunities:
\begin{itemize}\setlength{\itemsep}{0.cm}
\item {They provide a way to study nuclear modifications to PDFs and cold nuclear matter effects (such as shadowing, parton saturation, and energy loss) without the complexities of hot QCD medium effects present in AA collisions.}
\item {They serve as a crucial reference for disentangling initial-state nuclear effects from final-state medium effects in AA collisions, aiding in the interpretation of quark-gluon plasma (QGP) signatures.}
%due to the cleaner environment in which to studyy hadronisation and initial-state effects without significant final-state rescattering} 
\item {They typically achieve higher luminosities than AA collisions and reduced pile-up than in \pp\ collisions, allowing for more precise measurements.} 
\item {They provide a unique platform to extend studies of small-$x$ QCD and gluon saturation by probing smaller momentum fractions than any other current experimental setup.} %\Remark{CAF}{propose to add 'current', pp at 13.6 TeV or max 14 TeV at same rapidity would then be lower in x}
\item {They offer valuable insights
into the interplay of enhancement and suppression mechanisms in nuclear matter and a cleaner environment to study coalescence and fragmentation in hadronisation. } 
\item {They are essential for the modelling of high-energy cosmic-ray and neutrino interactions, providing a link between particle physics and astrophysics.}
%better testing ground for hadronic interactions in cosmic-ray physics} 
\end{itemize}

%It is instructive to recall that one of the scientific activities highlighted in the European Strategy for Particle Physics adopted by the CERN Council in xx directly concerned pA collisions 
%\begin{center}
%\begin{minipage}{0.9\columnwidth}
%9. A variety of important research lines are at the interface between particle and nuclear physics requiring dedicated experiments;
%\emph{Council will seek to work with NuPECC in areas of mutual interest, and maintain the capability to perform fixed target experiments at CERN.}
%\end{minipage}
%\end{center}

Through this contribution, our community emphasises the physics potential provided by the LHC beams --proton and heavy-ion-- in asymmetric \pA\ collisions, which offer multiple complementarities and advantages compared to \pp\ and AA collisions~\cite{Salgado:2011wc}. We summarise our physics case for a high-luminosity \pA\ run (HL-pA@LHC) under 12 topics, where large data samples are required to reduce the current experimental uncertainties and/or to study (for the first time) multiple rare processes of interest.
Our qualitative comparison of the impact that \pA\ can have on selected physics topics, with respect to other collision scenarios (EIC~\cite{AbdulKhalek:2021gbh}, FT@LHC~\cite{Hadjidakis:2018ifr}, pp@HL-LHC~\cite{Azzi:2019yne}, AA@HL-LHC~\cite{Citron:2018lsq}), is shown below with $\star$ symbols, and is discussed in detail throughout this document and in Refs.~\cite{Salgado:2011wc,Chapon:2020heu,Boer:2024ylx}.
%for a strong physics case motivating a complete HL  \pA\ run (dubbed $p$A@HL-LHC) for the LHC}. 
%This program should be understood with the four main LHC detectors, ALICE, ATLAS, CMS, and LHCb, as well as the small LHC detectors, LHCf, ...  
%\Remark{CAF}{not sure we discussed LHCf yet}
This writeup is based on recently published scientific papers, as well as oral contributions presented during a workshop at CERN on July 4-5, 2024 \href{https://indico.cern.ch/e/pA_LHC_2024}{https://indico.cern.ch/e/pA\_LHC\_2024}.

%In Sec.~\ref{acc}, we review technical beam and detector aspects before presenting our physics case in Sec.~\ref{case} together with selected flagship measurements. 
%It is then complemented by a brief discussion of additional ideas beyond these 9 subjects.

%\begin{table}[htpb!]\renewcommand{\arraystretch}{1.05}
\begin{table}[h]\renewcommand{\arraystretch}{1.05}
%\caption{Qualitative comparison, in our estimation, of various experimental setups. An increasing number of stars points indicates a better environment for researching a physics topic.  }
%We refer to~\cite{Hadjidakis:2018ifr,Boer:2024ylx,Citron:2018lsq,Chapon:2020heu,AbdulKhalek:2021gbh} for details.}
\label{tab:comp_qual}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{4.5cm}|c|c|c|c|c} %\hline
%   Physics topics \textbackslash Collider   & EIC~\cite{AbdulKhalek:2021gbh} & FT@LHC~\cite{Hadjidakis:2018ifr} & HL-pA@LHC & pp@HL-LHC~\cite{Azzi:2019yne} & AA@HL-LHC~\cite{Citron:2018lsq} \\ \hline \hline
Physics topics \textbackslash~Collider   & EIC & FT@LHC & HL-pA@LHC & pp@HL-LHC & AA@HL-LHC \\ \hline %\hline
PDFs
%\savefootnote{$\star\star\star$: no limitation;  $\star\star$: possible limitation;$\star$: data taking for special runs only} 
& $\star\star\star\star$ & $\star\star\star$ & $\star\star$ & $\star\star\star$ &  -- \\ \hline
%
nPDFs
%\savefootnote{$\star\star\star$: no impact on the other LHC experiments;  $\star\star$: no impact pending constraints; $\star$: significant impact} 
& $\star\star\star\star$ & $\star\star\star$  & $\star\star\star$ & -- & $\star\star$ \\ \hline
%
TMDs
%\savefootnote{$\star\star\star$: direct with small uncertainty;  $\star\star$: direct with moderate uncertainty;$\star$: indirect}  
& $\star\star\star$ & $\star\star\star$ & $\star\star\star$ & $\star\star$ & -- \\ \hline
nTMDs
%\savefootnote{$\star\star\star$: direct with small uncertainty;  $\star\star$: direct with moderate uncertainty;$\star$: indirect}  
& $\star\star\star$ & $\star\star$ & $\star\star$ & -- & $\star$ \\ \hline
%
GPDs
%\savefootnote{$\star\star\star$: highest ;  $\star\star$: high; $\star$: moderate [corresponding to 1 LHC year]}  
& $\star\star\star$ & $\star$  & $\star\star$ & $\star$ & -- \\ \hline
%
nGPDs
%\savefootnote{$\star\star\star$: highest ;  $\star\star$: high; $\star$: moderate [corresponding to 1 LHC year]}  
& $\star\star\star$ & $\star$  & $\star$ & -- & $\star\star$ \\ \hline
%
Parton saturation searches
%\savefootnote{$\star\star\star$: no limitation;  $\star\star$:  some target types are not possible; $\star$: only a few target types are possible} 
&  $\star\star\star$ & $\star$ & $\star\star\star\star$ &  $\star\star\star$ & $\star\star\star$ \\ \hline
%
Odderon searches
%\savefootnote{$\star\star\star$: no limitation;  $\star\star$:  some target types are not possible; $\star$: only a few target types are possible} 
&  $\star\star$ & $\star$ & $\star\star\star$ &  $\star\star$ & $\star\star$ \\ \hline
%
Parton collectivity & -- & $\star\star\star$ & $\star\star\star$ & $\star\star$ & $\star\star\star\star$ \\
 \hline
DPS/TPS & $\star$  & $\star$ & $\star\star\star\star$ &  $\star\star\star\star$ & $\star$ \\
\hline
%
Hadron spectroscopy
%\savefootnote{$\star\star\star$: highest; $\star\star$: high; $\star$: moderate}  
& $\star$ & $\star$ & $\star\star\star$ & $\star\star\star$ &  $\star\star$
%\savefootnote{with a redesigned E1096 target} 
 \\ \hline
%
BSM searches
%\savefootnote{$\star\star\star$: highest; $\star\star$: high; $\star$: moderate}  
& $\star$ & $\star$ & $\star\star$ & $\star\star\star\star$ & $\star\star$ 
%\savefootnote{with a redesigned E1096 target} 
 \\ \hline
\end{tabular}
}
\end{table}





%\clearpage


